Perturbing Isoradial Triangulations

We consider an infinite, planar, Delaunay graph which is obtained by locally deforming the embedding of a general, isoradial graph, w.r.t. a real deformation parameter $\epsilon$. This entails a careful analysis of edge-flips induced by the deformation and the Delaunay constraints. Using Kenyon's exact and asymptotic results for the Green's function on an isoradial graph, we calculate the leading asymptotics of the first and second order terms in the perturbative expansion of the log-determinant of the Beltrami-Laplace operator $\Delta(\epsilon)$, the David-Eynard K\"ahler operator $\mathcal{D}(\epsilon)$, and the conformal Laplacian $\underline{\Delta}(\epsilon)$ on the deformed graph. We show that the scaling limits of the second order {\it bi-local} term for both the Beltrami-Laplace and David-Eynard operators exist and coincide, with a value independent of the choice of initial isoradial graph. Our results allow to define a discrete analogue of the stress energy tensor for each of the three operators. Furthermore we can identify a central charge ($c$) in the case of both the Beltrami-Laplace and David-Eynard operators. While the scaling limit is consistent with the stress-energy tensor and value of the central charge for the Gaussian free field (GFF), the discrete central charge value of $c=-2$ for the David-Eynard operator is, however, at odds with the value of $c=-26$ expected by Polyakov's theory of 2D quantum gravity; moreover there are problems with convergence of the scaling limit of the discrete stress energy tensor for the David-Eynard operator. The bi-local term for the conformal Laplacian involves anomalous terms corresponding to the creation of discrete {\it curvature dipoles} in the deformed Delaunay graph; we examine the difficulties in defining a convergent scaling limit in this case. Connections with some discrete statistical models at criticality are explored.

==> reviewer-annex.tex <==
% !TEX encoding = UTF-8 Unicode
% !TEX root = ./perturbing.tex
\section*{For the reviewer}
\label{reviewerannex}


\medskip\noindent REPORT BY THE REVIEWER:


The manuscript addresses a model of discrete planar graphs under infinitesimal local perturbations. The main results are asymptotic expansions of the log-determinants of the laplacian, conformal laplacian, and the K\"ahler operator on such graphs. These quantities formally represent an energy density of the corresponding model defined formally using a path integral with a suitable Gaussian field (Grassmann field or Gaussian free field). David and Eynard have introduced in [DE14] a measure over triangulations of the plane pertaining to a discrete model for Quantum Gravity. The present manuscript by David and Scott studies this model at isoradial triangulations and their perturbations. In essence, isoradial triangulations correspond to flat space, while the perturbed triangulations give rise to non-trivial curvature and anomalies.

Specifically, the authors consider so called Delaunay graphs that can be regarded as generalizations of isoradial graphs. They use and generalize Kenyon’s methods and exact results [Ken02] on isoradial graphs for the determinants and Green’s functions of the aforementioned operators. More general Delaunay graphs arise from isoradial Delaunay graphs via (small) perturbations (by some discrete holomorphic function). The authors compute the expansion of the log-determinants of the laplacian and the K\"ahler operator under such perturbations. Notably the first-order variations of the operators only depend on the local geometry, while the second-order variations involve long-range effects as well. The authors in particular find the cross-terms in a certain bilocal perturbation, 
and also consider scaling limits of these formulas and note that these agree (moreover with a value independent of the choice of initial isoradial graph). The perturbation should be small enough for the results to hold.

In contrast, for the conformal laplacian the situation is different: the bi-local perturbation of its determinant involves anomalous terms arising from curvature effects. It is not clear how to derive a scaling limit for the quantities involving the conformal laplacian. In an appendix, the authors present scaling limits of the anomalous terms for the deformation of the conformal laplacian, that are argued to reflect the global geometry. (They present there several formulas whose interpretation however remains unclear at least to me.)

The authors also define discrete analogues of the stress energy tensor (SET) for each three operators. At the level of central charges, this matches with $c = -2$, as it should for the laplacian. The authors however point out that they would expect that the K\"ahler operator also gives rise to Polyakov’s theory of 2D quantum gravity with $c = -26$; this possible connection seems to remain quite unclear. The authors speculate that the lack of relationship with Polyakov’s theory may be caused by problems with the convergence of the scaling limit for the SET of the K\"ahler operator. Regarding scaling limits, of the three operators only for the Laplace-Beltrami operator the associated discrete SET has an interpretation in the scaling limit in a QFT either in a free bosonic theory, or alternatively in terms of a free complex Grassmann field.

The paper seems interesting but not carefully written. Many definitions and easy geometric facts are clearly stated, but more involved arguments are sometimes only sketched and sometimes omitted completely. In the current presentation, it is not possible to fully follow the arguments. Hence the presentation should be significantly improved, interesting observations should be highlighted, in the technical parts the main ideas should be clarified, proofs should be added, and some more background would also be useful to the readers. Moreover, several typos and incorrect references should be fixed. The potentially interesting results of the paper are at the moment hidden under poorly explained technical details, and one cannot be convinced of their validity.

\color{blue}
\medskip
\noindent REPLY OF THE AUTHORS:

\medskip
\noindent 
We thank the reviewer for his careful reading of the manuscript and his perceptive comments. We tried to take them into account in this revised version of the paper. 
We added the missing figures and proofs, and extended the arguments which were found sketchy by the reviewer. 
In addition, we added background material, explained our motivation for this work, and highlighted the new results and interesting observations in the introduction, and in the beginning of the technical sections.
We also added references.

\medskip
\noindent  The abstract is fully rewritten.

\medskip
\noindent The introduction (Sect.~\ref{sIntro}) is extensively rewritten.

Subsection 1.1 is an entirely new presentation which includes the motivation for our work, its connection to 2d gravity, as well as the key points addressed in the article. It supersedes subsections 1.1 and 1.3 of the first version, with a lot of more material, including the points which in the the first version were present only in the concluding section 9.

Subsection 1.2 is expanded and presents: (i) the geometrical concepts and tools (1.2.1), (ii) the random triangulation model, (iii) the operators .

Subsection 1.3 present the main results of the paper and replaces the subsection 1.4 of the first version. Some important technical results not presented in the previous version are now discussed, as well as results about the discrete stress energy tensors and its connections with CFT's.

\medskip
\noindent The questions and comments of the referee in Section 2, 3 and 4 have been taken into account.
In Section 3, the distinction between triangulations, Delaunay graphs, and critical graphs (Delaunay isoradial graphs) has been made clearer.

\medskip
\noindent The section 5 has been reorganized, and its title has been changed.

We first discuss the geometry of deformation of graphs (in Sect. 5.1 and 5.2) and in particular we introduce the notion of stable deformation (in Def. \ref{StableDef}) to make clear the difference between Delaunay deformations (with Lawson's flips) from deformations without flips (stable). The bounds on the deformation parameter $\epsilon$, which ensures that a Delaunay deformation is stable (in our new langage), previously in sect. 5.4, are now in sect. 5.2, and the formulation and the proofs have been improved.

The results and the discussion for the first order deformation of the operators, previously in sect. 5.1 and 5.2, are now in sect. 5.3 and 5.4.

\medskip
\noindent In section 6, and 7, we better organized the sections through new subsections for each separate points discussed, and we took into account the questions and comments of the referee.

\medskip
\noindent Section 8, which contains most of the technical results, has been revised. We took into account the remarks of the referee. When needed, the results have been stated more precisely, and details have been added to the proofs to make them clearer.

Subsection 8.1 has been expanded ans now presents a detailed introduction and outline of the questions which are addressed there. It should make the logic and organisation of this section clearer.

Subsection 8.2 has been revised, taking into account the definition of rigid deformation introduced in section 5.  It should be clearer now.

Subsections 8.3 -- 8.6 are better organized.

Subsection 8.7 about the scaling limits for $\Delta$ has been split into two subsections.

\medskip
\noindent The questions and comments of the referee in the concluding section 9 have been taken into account. We hope that the discussion in subsection 9.3 is clearer, in view of the new material in the introduction, especially subsection 1.1.

\medskip
\noindent 
In Appendix A we have added a subsection about the conformal ghost-antighost $\mathbf{b}-\mathbf{c}$ theory.

\medskip
\noindent In Appendix C, Claim 1 is now Lemma 16 and we added a proof. Claim 2 is now a Proposition.


\medskip\noindent REPLY TO THE SPECIFIC COMMENTS:

\color{black}
\medskip\noindent Some comments:
 
\medskip\noindent
 1. In the text, there are some typos and grammatical errors here and there (especially singular/plural). I’m not going to list all of them here.
 
\color{blue} \medskip
 Thank you, we did our best to locate and correct them.

\color{black} 
\medskip\noindent
2. Also the bibliography contains typos e.g. in the authors’ names. 

\color{blue}\medskip
 Thank you, we did our best to locate and correct them.

\color{black} 
\medskip\noindent
3. In the abstract you mention problems for convergence in the scaling limit of the SET associated to the K\"ahler operator; how about the conformal laplacian?

\color{blue}\medskip
For the conformal Laplacien no term for the OPE has a scaling limit. This is better discussed in the paper.
 
\color{black} 
\medskip\noindent
4. eq.(1.3): why anti-holomorphic? Also, what is F supposed to be here?

\color{blue}\medskip
This is better explained in the text and in appendix \ref{ssT2DCFT}
 
\color{black} 
\medskip\noindent
5. p5: explicitely -> explicitly

\color{blue}\medskip
Corrected
 
\color{black} 
\medskip\noindent
6. p5: What is the distinction of the critical laplacian and the Laplace- Beltrami in eq.(1.1)? You denote both as $\Delta$. The notation and definition should be clearer. Also the discrete $\partial$, $\bar\partial$ are not defined.

\color{blue}\medskip
This is explained, see Rem. 7.
 
\color{black} 
\medskip\noindent
7. Also in (1.7) the difference of the discrete $\Delta$ and $\Delta_{\mathrm{cr}}$ should be explained there. On page 9 the definition 
of $\Delta_{\mathrm{cr}}$ is not clear.

\color{blue}\medskip
The distinction between $\Delta_\text{cr}$ (referring to isoradial Delaunay graphs) and $\Delta$ (referring to general Delaunay graphs) is now made more precise in the Introduction \ref{sIntro}, see definition \ref{crDeltaDef}, as well as in section \ref{sLaplacians}, see definition \ref{critlaplacian}.
 
\color{black}\medskip\noindent
8. p5, Fig 1: It seems here and in a few other places that the manuscript is not ready for submission.

\color{blue}\medskip
Sorry for the omission. This is corrected
 
\color{black}\medskip\noindent
9. eq.(1.6): what are z1, z2, z3? The definition of the measure is not clear.

\color{blue}\medskip
This is now explained.
 
\color{black}\medskip\noindent
10. end of p5: Explain why non-triangulations have measure zero.

\color{blue}\medskip
This is now explained.
 
\color{black}\medskip\noindent
11. p8: where is lemma 1 proven?

\color{blue}\medskip
Lemma 1 is now Prop.~\ref{LemmaOne}. Where it comes from is now stated. 

\color{black}\medskip\noindent
12. Does Proposition 10 imply theorem 1? It would be good to say so after the statement of thm.1. 

\color{blue}\medskip
Yes, the theorem has been rewritten, and where it comes from is stated explicitly in the text.

\color{black}\medskip\noindent
13. Does Proposition 11 imply theorem 2? It would be good to say so after the statement of thm.2. 

\color{blue}\medskip
Proposition 11 is now part of Theorem 1.

\color{black}\medskip\noindent
14. thm.2: You write “In particular, $c = -2$” but the asymptotic (1.15) does not show this. 

\color{blue}\medskip
This is explained now in Section~\ref{sssIntroTC} of the introduction.

\color{black}\medskip\noindent
15. above lem 2: appendix B (not A); please make sure that the references are correct 

\color{blue}\medskip
This is corrected.

\color{black}\medskip\noindent
16. lem 2: Can you motivate the constants 3/2 and 1/2 here? 

\color{blue}\medskip
Not really. They are just technical coefficients coming out of the detailed derivation. They can be probably improved, but this is not important.

\color{black}\medskip\noindent
17. Remark 2: Green’s theorem is LEMMA 4, not THM 4. 

\color{blue}\medskip
This is corrected.

\color{black}\medskip\noindent
18. p11: where is Proposition 1 proven? 

\color{blue}\medskip
This is now explained. 

\color{black}\medskip\noindent
19. p14: Is Prop.20 using Conj.1? 

\color{blue}\medskip
Yes, this is stated in the text.

\color{black}\medskip\noindent
20. p16: embedding -> embedded 

\color{blue}\medskip
This is corrected.

\color{black}\medskip\noindent
21. (2.1): Should the cross-ratio here have absolute values? 

\color{blue}\medskip
No, the correct definition is indeed \ref{ConfAngleDef}.

\color{black}\medskip\noindent
22. p17: remark 9: in the case $\theta_n(e) = - \theta_s(e)$ it seems to me that both are zero. Please explain. 

\color{blue}\medskip
No, they are in general non-zero. This is discussed more in remark \ref{Rem9}.

\color{black}\medskip\noindent
23. p17: Should the cross-ratio here have absolute values? 

\color{blue}\medskip
No.

\color{black}\medskip\noindent
24. p18, top: there are too many words “discussion” 

\color{blue}\medskip
This is corrected

\color{black}\medskip\noindent
25. eq.(2.3): You could explicate the curvature also in fig. 4. 

\color{blue}\medskip
The caption of the figure has been rewritten.

\color{black}\medskip\noindent
26. p22: fig. 2.2 does not exist. 

\color{blue}\medskip
This is corrected. It is now fig.~\ref{asymptotic-train-track-1}

\color{black}\medskip\noindent
27. p23: Where is the proof of Prop.2? 

\color{blue}\medskip
The proposition has been removed since it is redundant.
Its statement is part of  Prop.~\ref{semi-circle-property}. Its proof is given.

\color{black}\medskip\noindent
28. p26: figure 11 is missing. 

\color{blue}\medskip
The missing figure is not useful and has been removed.

\color{black}\medskip\noindent
29. remark 14: the end should read “for any function $\phi \in \dots$” 

\color{blue}\medskip
This is corrected

\color{black}\medskip\noindent
30. p30: It would be good to recall the definition of $A(\mathrm{x})$. 

\color{blue}\medskip
This has been added.

\color{black}\medskip\noindent
31. p30: Where is the proof of lemma 4?

\color{blue}\medskip
The proof has been added.

\color{black}\medskip\noindent
32. Remarks 15-16: It would be good to include a more detailed reference for these local identities. 

\color{blue}\medskip
The references and details have been added.


\color{black}\medskip\noindent
33. p31: (3.17) should include “for all $\psi \in \Bbb{C}^{\mathrm{F}(\uG)}$"

\color{blue}\medskip
This have been added.

\color{black}\medskip\noindent
34. p31, Sect.3.3: It would be useful to relate the definitions of the determinants to Kenyon’s work. 

\color{blue}\medskip
This is explained after Eq. \ref{limit-normalized-reduced}.

\color{black}\medskip\noindent
35. p32: What is “discussion in 1”? 

\color{blue}\medskip
The reference has been removed.

\color{black}\medskip\noindent
36. p32: the equation after (3.21) should have for some (not all) $a, b \in \Bbb{Z} $

\color{blue}\medskip
This is true for all $a,b$, but $m,n$ fixed . This has been corrected.

\color{black}\medskip\noindent
37. p32: , and consequently... 

\color{blue}\medskip
This is corrected

\color{black}\medskip\noindent
38. (3.23): Why does the limit exist? 

\color{blue}\medskip
This is now explained (heuristically).

\color{black}\medskip\noindent
39. (3.24): subscripts “n” are missing 

\color{blue}\medskip
This is corrected

\color{black}\medskip\noindent
40. (3.24): is $K$ supposed to be an integer? 

\color{blue}\medskip
Yes. This is corrected

\color{black}\medskip\noindent
41. p33: the reference to (5.1) seems out of place, rather refer to an earlier equation or give the formula here 

\color{blue}\medskip
Yes. \ref{zPertF}  is replaced by \ref{thezdeform}

\color{black}\medskip\noindent
42. (3.27, 3.29): I don’t think the notations used here are defined: $V_{\scriptscriptstyle 11}$, $\cyrLL$, $\mathcal{L}$. (Admittedly 
$\cyrLL$ comes in (3.30) but it’s impossible to know this when looking at the previous subsection where (3.27) appears.) 

\color{blue}\medskip
Yes, the notations are recalled after Eq. \ref{kenyon-log-det}

\color{black}\medskip\noindent
43. p34: For a chord, it seems again that $\theta_{\mathrm{n}}(\ue) = -\theta_{\mathrm{s}}(\ue) = 0$, is this correct? 

\color{blue}\medskip
No, this is explained before.

\color{black}\medskip\noindent
44. p35: chosen 

\color{blue}\medskip
This is corrected

\color{black}\medskip\noindent
45. p35: what is formula (12)? 

\color{blue}\medskip
This is corrected

\color{black}\medskip\noindent
46. fig.14 should have an explanation and this should be used to clarify the statement of Remark 20. 

\color{blue}\medskip
Fig. 14 is replaced by Fig.~\ref{Cocyclic-1-TX}  and its caption explains the statement.


\color{black}\medskip\noindent
47. p41: Recall from (4.9) what $\frak{u}$ is. 

\color{blue}\medskip
This has been added.

\color{black}\medskip\noindent
48. p41: What does “bounded by 5” in prop.4 mean? 

\color{blue}\medskip
This is explained in Lemma~\ref{lemma-p-estimate}.

\color{black}\medskip\noindent
49. p43: Can you explain the geometric meaning of (5.5)? 

\color{blue}\medskip
Unfortunately no. It comes out from the calculation.

\color{black}\medskip\noindent
50. p44: what is Appendix 8? Give the formula for (5.8) here.

\color{blue}\medskip
The Appendix was a Section. The formula has been written explicitly

\color{black}\medskip\noindent
51. p44: similarily -> similarly 

\color{blue}\medskip
This is corrected

\color{black}\medskip\noindent
52. What is the meaning of eq.(5.12)-(5.14)? 

\color{blue}\medskip
The meaning of these equations is now explained.

\color{black}\medskip\noindent
53. p46: Lawson edge flips have not been defined.

\color{blue}\medskip
They are now defined. 

\color{black}\medskip\noindent
54. p46: How are the deformed edges defined? It’s not clear to me that the deformed vertex set determines a Delaunay graph or even a polyhedral graph. 

\color{blue}\medskip
This is now extensively discussed. 

\color{black}\medskip\noindent
55. p47 \& 51: What is Appendix 8? 

\color{blue}\medskip
This is corrected

\color{black}\medskip\noindent
56. p47: ensure 

\color{blue}\medskip
This is corrected

\color{black}\medskip\noindent
57. p48: cross-ratio 

\color{blue}\medskip
This is corrected

\color{black}\medskip\noindent
58. p49: many -> may 

\color{blue}\medskip
This is corrected

\color{black}\medskip\noindent
59. p49: for for 

\color{blue}\medskip
This is corrected

\color{black}\medskip\noindent
60. Prop.7 has “Laplace” two times. 

\color{blue}\medskip
The reference is corrected

\color{black}\medskip\noindent
61. Could you add an argument why Remark 29 is true? 

\color{blue}\medskip
This is added.

\color{black}\medskip\noindent
62. Prop.8: it would be good to recall the notation  $\cyrLL(\theta)$ in (6.6). 

\color{blue}\medskip
We put a  reference back to formula \ref{lobachevsky} where the Lobachevsky function is defined.

\color{black}\medskip\noindent
63. p64: Theorem 10 does not exist. 

\color{blue}\medskip
This is corrected

\color{black}\medskip\noindent
64. p64: What is proof 6.1 ? 

\color{blue}\medskip
The reference has been added.

\color{black}\medskip\noindent
65. p64, bottom: G0+ appears too many times between (6.52) and (6.53) 

\color{blue}\medskip
This is corrected

\color{black}\medskip\noindent
66. p70: What does $(\varepsilon0, \pi, 0, \pi)$ ! mean? 

\color{blue}\medskip
This was a typo. It is corrected

\color{black}\medskip\noindent
67. p70: saclar -> scalar 

\color{blue}\medskip
This is corrected

\color{black}\medskip\noindent
68. p73: factor factor 

\color{blue}\medskip
This is corrected

\color{black}\medskip\noindent
69. p77: become 

\color{blue}\medskip
This is corrected

\color{black}\medskip\noindent
70. p80: leads, or will lead 

\color{blue}\medskip
This is corrected

\color{black}\medskip\noindent
71. p80: Is Prop.20 using Conj.1? 

\color{blue}\medskip
This is specified in the proposition (now Prop.~\ref{PropLimTr2D}).

\color{black}\medskip\noindent
72. p80: Where does (8.2) follow from? 

\color{blue}\medskip
This is now explained.

\color{black}\medskip\noindent
73. p81: I’m not able to follow the text between (8.3) and (8.4). Please explain and illustrate the meaning of the back-deformation. 

\color{blue}\medskip
Indeed there was some error in the notations, which confused the discussion. This part has been rewritten. We hope it is now clear.

\color{black}\medskip\noindent
74. p84: In the second line or subsect.8.5 the notations after $A_\epsilon$, $R_\epsilon$ are not correct. 

\color{blue}\medskip
Indeed. This has been corrected.

\color{black}\medskip\noindent
75. p85: has $R_0$ been defined?

\color{blue}\medskip
Yes, at the beginning of sect. \ref{ssFullVarFlip} and later again at the beginning of Sect.~\ref{sssBndDiscrDer}.
 

\color{black}\medskip\noindent
76. p87, prop. 12 (proof): This is not acceptable. Please finish the manuscript
before sending it to be referee.

\color{blue}\medskip
Sorry, we omitted to write the proof. The discussion leading to the proposition has been simplified, the proposition rewritten, and the detailed proof added.

\color{black}\medskip\noindent
77. p88: The procedure 8.4 is not really clear, please explain and illustrate its meaning. 

\color{blue}\medskip
The procedure is explained more clearly in the rewritten section, now \ref{ssFlipsNoFlips}

\color{black}\medskip\noindent
78. p88: Fig ?? 

\color{blue}\medskip
The figures are quoted correctly now

\color{black}\medskip\noindent
79. p88: in other words 

\color{blue}\medskip
This has been corrected.

\color{black}\medskip\noindent
80. Where is the proof of prop.14? 

\color{blue}\medskip
The proof of the proposition (now Prop.~\ref{PropLimDpr}) has been added.

\color{black}\medskip\noindent
81. The text beneath (8.69) is not clear.

\color{blue}\medskip
The text has been simplified. 

\color{black}\medskip\noindent
82. p92: What is Pro.8.66? 

\color{blue}\medskip
It was an equation. This is corrected.

\color{black}\medskip\noindent
83. It would be good to clarify the notations in (9.1). It is very hard to remember all notations here. 

\color{blue}\medskip
We have added the references for the notations in equations \ref{varTrLlLB3} and \ref{Kexplicit}.

\color{black}\medskip\noindent
84. p96: In the equation above (9.3) it would be useful to switch the order of the terms involving $\overline{\partial} F$ and $\partial \overline{F}$ to accommodate with the analogy in the discrete equation above, where only $\overline{\nabla} F$ is shown and the other term is written as c.c. (Also, eq.(9.3) seems unnecessary to me, as the analogy is already explained in the text. There are many other places in the manuscript where clarifications would be needed, while this is not one of those.) 

\color{blue}\medskip
We have switched the order of the two terms. We prefer however to keep \ref{Discr2Cont}.

\color{black}\medskip\noindent
85. p98: at variance -> in contrast 

\color{blue}\medskip
This is corrected.

\color{black}\medskip\noindent
86. p99, 2/3: than -> as 

\color{black}\medskip\noindent
87. p99: “which a simple” seems misplaced 

\color{blue}\medskip
The paragraphs after \ref{TconfDiscrSchem} has been rewritten and simplified. Rem. 86 and 87 are not relevant anymore.

\color{black}\medskip\noindent
88. p100: What is Proposition 5.3? 

\color{blue}\medskip
This is corrected.

\color{black}\medskip\noindent
89. p101: variatioN 

\color{blue}\medskip
This is corrected.

\color{black}\medskip\noindent
90. p101: for for 

\color{blue}\medskip
This is corrected.

\color{black}\medskip\noindent
91. p101: You mention Polyakov’s theory here and speculate a relation with Fadeev-Popov determinant. It would be nice to include a discussion about Fadeev-Popov ghosts e.g. in Appendix A where you already discuss QFT aspects. Why is a relation to be expected? 

\color{blue}\medskip
A discussion about  Fadeev-Popov ghosts has been added in Appendix A  in Sect.~\ref{AppBCsystem}. Ghosts are also discussed in the Introduction, which has been extensively rewritten.

\color{black}\medskip\noindent
92. Also, it seems that only around page 101 you really explain what are the main results of the paper and why they are interesting. You cannot expect readers to make it through 100 pages of technical work before motivating the results. It would be better to include more motivation and ideas of the work in the introduction. 

\color{blue}\medskip
The Introduction has been extensively rewritten. It includes more motivation and ideas of the work in \ref{ssIntPurpMot}. It also presents and discusses more extensively what are the important results in \ref{ssResults}.


\color{black}\medskip\noindent
93. p105: Virasoro (several occasions) 

\color{blue}\medskip
This is corrected.

\color{black}\medskip\noindent
94. p109: Please explain how (A.11) and (A.12) are not unrelated. 

\color{blue}\medskip
This is now explained.

\color{black}\medskip\noindent
95. bottom of p110: some parentheses are misplaced around Berezin integral in the text 

\color{blue}\medskip
This is corrected.

\color{black}\medskip\noindent
96. p116: Refer to fig.33 for illustration of $\uG_\mathrm{cr}$ in the text. 

\color{blue}\medskip
This is corrected.

\color{black}\medskip\noindent
97. p116: What is Claim ?? ? 

\color{blue}\medskip
This is corrected into a reference to Prop.~\ref{epsilontildeF}

\color{black}\medskip\noindent
98. p116: of of 

\color{blue}\medskip
This is corrected.

\color{black}\medskip\noindent
99. p118: Is Claim 1 going to be proven, or is it taken as an assumption? 

\color{blue}\medskip
Claim 1 is now Lemma~\ref{uniform-convergence}, with a proof. 

\color{black}\medskip\noindent
100. p119: where where 

\color{blue}\medskip
This is corrected.

\color{black}\medskip\noindent
101. Appendix C: can you interpret the formulas in Claim 2?

\color{blue}\medskip
There is no simple interpretation of these formulas now in Prop.~\ref{continuum-limits-anomalies}, which come out of the calculation, we are afraid.

\color{black}


